Unleashing the Power of Emojis in Texts via Self-supervised Graph Pre-Training

Emojis have gained immense popularity on social platforms, serving as a common means to supplement or replace text. However, existing data mining approaches generally either completely ignore or simply treat emojis as ordinary Unicode characters, which may limit the model's ability to grasp the rich semantic information in emojis and the interaction between emojis and texts. Thus, it is necessary to release the emoji's power in social media data mining. To this end, we first construct a heterogeneous graph consisting of three types of nodes, i.e. post, word and emoji nodes to improve the representation of different elements in posts. The edges are also well-defined to model how these three elements interact with each other. To facilitate the sharing of information among post, word and emoji nodes, we propose a graph pre-train framework for text and emoji co-modeling, which contains two graph pre-training tasks: node-level graph contrastive learning and edge-level link reconstruction learning. Extensive experiments on the Xiaohongshu and Twitter datasets with two types of downstream tasks demonstrate that our approach proves significant improvement over previous strong baseline methods.

==> latex/2related2.tex <==

\section{Related Work}
\label{sec:related}

%Emojis are graphical symbols or ideograms commonly known as ``picture characters''. They serve as visual representations that can convey a broad range of concepts and ideas. Emojis are widely used to depict not only facial expressions and emotions but also various non-emotional meanings such as celebrations, weather conditions, transportation and buildings, food and beverages, animals and plants, and diverse activities. Due to the remarkable ability to convey rich semantics, which express ideas and emotions in a vivid manner,  emojis are extensively utilized in online communication across various digital platforms and contexts, particularly on social media.  What's more, some standards of emojis, \emph{e.g.}, the Unicode standard, ensure that emojis can be seamlessly used without language barriers among people from different countries.  Given their widespread usage, emojis have become a subject of extensive research, ranging from analyzing user preferences to studying their impact on digital marketing and sentiment analysis~\citep{Gandhi2022, Chen2019}.

Emojis serve multiple purposes in communication, encompassing 1) conveying emotions or situational information to add meaning to the message, 2) adjusting the tone of the communication, and 3) acting as a social tool to engage recipients, facilitating socially acceptable conversations, and supporting relationship maintenance \citep{cramer2016sender}. However, empirically, the role of emojis in textual content comprehension is complicated. The majority of the existing literature found a complementary role of emojis in textual content. \cite{boutet2021emojis} demonstrated that emojis enhance digital interactions by conveying information about the sender's affect and personality traits, and the inclusion of a congruent emoji can enhance the processing of verbal messages. \cite{hand2022interactions} discovered that sentence valence and emoji type interact to influence message emotionality, clarity, and perceived sender warmth and state. \cite{logi2021social} applied an analytical framework to explore the meaning of emojis both individually and in interaction with language. \cite{pfeifer2022all} found that all facial emojis impact text processing, with happy and upset emojis carrying differential social-emotional salience and affecting text processing when content becomes available. \cite{volker2021tuned} demonstrated that emojis provide cues to extract emotional information from text-based messages, and emotionally intelligent recipients appear particularly responsive to them. This body of research illuminates the captivating and intricate role of emojis in complementing texts, thereby enhancing both textual comprehension and emotional expression.

However, the role of emojis goes beyond mere complementing of texts; they also serve as substitutes for words within texts. \cite{cohn2018emoji} conducted research revealing that replacing words with images in sentences incurred a processing cost in terms of self-paced reading times. Interestingly, verb emojis placed in noun positions exhibited even longer reading times compared to standard emojis. Building on these insights, \cite{cohn2019grammar} highlighted that emojis were more frequently employed as substitutions for nouns and adjectives rather than verbs. This nuanced usage often conveyed nonredundant information within sentences. \cite{orazi2023non} ventured into the realm of multiple substitutive emojis in a message, revealing that such utilization hindered processing fluency, consequently impacting message evaluations and electronic word-of-mouth (eWOM) volume. Despite these findings, \cite{scheffler2022processing} demonstrated that sentence comprehension remains intact even when emojis replace words.

In certain scenarios, emojis neither complement nor replace words; rather, they can contradict the intended meanings of words or sentences. \cite{chen2018twitter} introduced an innovative framework for Twitter sentiment analysis, spotlighting emojis with a focus on contradictory semantics or sentiments that often convey intricate nuances such as irony and sarcasm. \cite{hand2022interactions} uncovered that incongruent emojis diminished message clarity compared to situations involving no emoji or congruent ones. Echoing this, \cite{yang2022effect} observed that emojis primed with emotional content congruent with subsequent words facilitated linguistic information processing, while those featuring incongruent emotional content hindered comprehension. \cite{beyersmann2022s} shed light on the interpersonal dynamics enhanced by congruent emojis, as separate ratings indicated that message senders who included congruent emojis were more favorably received than those using incongruent ones. Crucially, when the contents of an emoji and a text are incongruent, the text takes precedence over the emoji \citep{wang2014effects}. In a similar vein, \cite{derks2008role} noted that individuals tended to prioritize the verbal aspects of communication when the meanings of textual messages clashed with those conveyed non-verbally. In essence, if the verbal message was negative, even an inserted positive emoticon wouldn't alter the overall perceived negative tone.

\subsection{Emojis in Natural Language Processing}

Currently, many researchers have not fully realized the importance of emojis in their textual studies~\citep{mikolov2013efficient,hotho2005brief,allahyari2017brief}. Only some recent works have begun to focus on the significance of emojis, and these can be summarized into the following four lines of research.

\hide{Due to the undeniable rapid trend of emojis, many NLP researchers have taken notice and conducted various related studies, resulting in significant progress. These studies can be primarily categorized into four types: traditional processing methods, studies on representing emojis with text information, supervised learning, and self-supervised learning.

In the current field of natural language processing, the prevailing method have received very little training on the use of emojis, resulting in emojis often being identified as the unknown token ($<$unk$>$) by the language models even when they are correctly segmented.
This limited recognition of emojis by the language models reduces the potential benefits for downstream tasks. 
Due to the variety of emojis, many emojis are difficult to be tokenized.
}
% \vpara{1. Traditional Processing Methods.}

% standard pre-processing.
% Given this situation, the traditional methods for processing emoji information in natural language can be primarily divided into the following four categories: 
% (3)  {\textit{Replacing emojis with words}:} This method replaces emojis with specific words or symbols; for example, replacing ``\emoji{smiley}'' with ``smile''. 
The first line of works directly utilizes some standard pre-processing methods to handle emojis, and then feed the pre-processed emojis to language model~\citep{pavan2019novel,Wijeratne2017,Yinxia2020}. Specifically, 
(1) {\textit{Removing emojis}:} This method involves removing emojis from the text, treating them as noise, but it ignores the semantic information conveyed by emojis~\citep{pavan2019novel}.
(2) {\textit{Keeping emojis}:} This method retains emoji as a token, but unfortunately, the token cannot convey the meanings carried by the emoji~\citep{Yinxia2020}.
(3)  {\textit{Translating emojis into text}:} This method translates emojis with descriptive text~\citep{Wijeratne2017}; for example, replacing ``\emoji{smiley}'' with ``smile''. 
However, this necessities a dictionary that can only covers specific types of emojis (\emph{e.g.}, iOS emojis encoded by Unicode) and cannot include other types of emojis (\emph{e.g.}, Xiaohongshu emojis and user-created emojis), as
the example illustrated in Table~\ref{tab:limitations} (a).
Besides, these approaches completely cannot tell a sentence with emojis from that without emojis, as shown in Table~\ref{tab:limitations} (b).
% eliminate the structural relationship between text and emojis. This makes it impossible to distinguish between text with
% and without emojis. Tab
% However, these methods have limitations as they do not fully consider the semantic information conveyed by emojis, resulting in limited benefits for NLP tasks.

\begin{table}[]
  \caption{Two main limitations of standard pre-processing methods to handle emojis: limited coverage range and loss of emoji pattern.}
  \label{tab:limitations}
  \centering
  \setlength{\fboxsep}{0pt} % Remove padding around the image
  \begin{tabular}{c}
    \includegraphics[width=\linewidth]{figures/emojilimitations.pdf} \\
  \end{tabular}
\end{table}

% \citep{Wijeratne2017}This category involves applying existing NLP techniques to handle emojis. There are three main approaches:
%  i) Direct removal of emojis.
%  ii) Treating emojis as special characters or symbols within text data.
%  iii) Converting emojis into textual representations for processing.

% \vpara{2. Studies on Representing Emojis with Text Information:} 
To distinguish a sentence with emojis from that without emojis, another line of research explores ways to learn emoji representations by utilizing the textual description associated with emojis~\citep{Eisner2016emoji2vecLE}. This approach learns emoji representations by minimizing the similarity between the representations of emoji and its textual description. However, it relies on the availability of textual descriptions for emojis, which may not always be accessible for certain emojis, such as user-created emojis.
% \JR{~\citep{Yinxia2020} introduce an attention model to jointly learn emoji representation and text representation by a sentiment classification task.??} 
% they all rely on the textual description of emojis, while the textual description of many emojis, like  user-created emojis, is inaccessible in some cases.
% those user-created emojis usually have no textual descriptions.

% \vpara{3. Supervised Learning:} 

The third line of works utilizes emojis to help certain tasks, \emph{e.g.}, sentiment classification, emotion analysis, emoji prediction~\citep{Chen2019,singh-etal-2022-emoji,zhao2023pedm}. For example, ~\citep{Chen2019} addresses cross-lingual sentiment classification by employing emojis as an instrument, because similar emojis express similar emotions across different language contexts.  However, these approaches can only leverage the emoji meaning related to certain task at hand; \emph{e.g.}, emojis employed for sentiment classification may not effectively represent the semantic and concrete meaning of an emoji like ``\emoji{car}''.

% cannot represent semantic and concrete meaning in emoji ``\emoji{car}''.
% represent only the sentiment meaning of the emoji, but 
% cannot represent semantic meaning.

% involves training models using labeled data, where the relationship between text and emojis is explicitly provided~\citep{Chen2019,singh-etal-2022-emoji,zhao2023pedm}. Researchers create annotated datasets where text inputs are paired with corresponding emojis, allowing models to learn the association between specific textual contexts and the appropriate emoji representation.

% \vpara{4. Self-Supervised Learning:} 
Approaching emoji information suitable for different tasks and capable of conveying richer meanings, the fourth line of works in the literature explores leveraging self-supervised or unsupervised tasks to utilize emoji information or learn emoji representations.
For example, \citep{deepmoji,park-etal-2018-plusemo2vec}  design a self-supervised task to identify whether a post contains certain emoji so as to incorporate emoji information into text representations. Another work, \citep{emojicoocurrence}, constructs an emoji co-occurrence network and learns emoji representations by minimizing the similarity between neighboring emojis. 
% \JR{However, the limitation of these approaches is that they neither consider the position nor the relation between text and emojis. Our study addresses this research gap by exploring methods that incorporate the position and relation between text and emojis.}

% that two posts with similar emojis 
% nor the emoji's text context (i.e., words around the emoji)

% do not consider the emoji's text context (i.e., words around the emoji), which often provides rich and valuable information. Ignoring the contextual information may lead to the loss of important nuances and potential ambiguity in emoji meanings. To address this limitation, future research could explore methods that incorporate the text context surrounding emojis, enabling more comprehensive and contextually aware emoji representations suitable for a broader range of natural language processing tasks.

% the emoji's text context (\emph{i.e.}, words around emoji) provides rich information, none of these works take it into consideration.
 
% \JR{Self-supervised learning aims to learn representations without relying on explicit annotations. In the context of emojis, this approach involves leveraging large amounts of unlabeled text data to learn the underlying structure and patterns related to emojis. Techniques such as language modeling or pre-training are employed to capture the inherent semantic relationships between text and emojis. Self-supervised learning requires no manual annotation and can effectively learn emoji and text representations. Fine-tuning these models can yield promising results for various downstream tasks. For example, the work on \citep{deepmoji} collects a large amount of text data containing emojis, designs a text-emoji prediction task to incorporate emoji information into text, and applies the learned representations to other downstream tasks through transfer learning. Similarly, \citep{park-etal-2018-plusemo2vec} uses clustering algorithms to group emojis into different clusters and employs self-supervised learning by predicting the emoji cluster for a given text, thereby capturing information related to similar emojis. Another work, \citep{emojicoocurrence}, constructs a graph network based on the co-occurrence of emojis in posts and learns emoji representations by minimizing the similarity between neighboring emojis. However, this work overlooks the semantic context of the text.

% In this study, a bipartite graph network is constructed to capture the relationships between posts and emojis. Two self-supervised learning tasks are designed: node-level subgraph contrastive learning and post-emoji link prediction. These tasks enable the joint learning of post and emoji representations, extracting richer information from both the text and emojis. The effectiveness of the proposed method is validated through two downstream tasks.
% }

% \hide{
% In the current field of natural language processing, the prevailing method involves fine-tuning pre-trained large language models to adapt to a variety of downstream tasks. However, these models have received very little training on the use of emojis, resulting in emojis often being identified as the unknown token (<unk>) by the language models even when they are correctly segmented. This limited recognition of emojis by the LLMs reduces the potential benefits for downstream tasks. Furthermore, due to the variety of emojis, many of them are difficult to tokenize under standard pre-processing, and may require separate extraction and processing. Given this situation, the current methods for processing emoji information in natural language processing tasks can be primarily divided into the following four categories: 

% \begin{itemize}
%     \item {\bfseries{Delete:}} Remove emojis from text, treating them as noise.
%     \item{\bfseries{Keep:}} Keep emojis in text and directly use LLM to learn it.
%     \item{\bfseries{Replace:}} Replace emojis with specific words or symbols, e.g., replace ``\emoji{smiley}" with ``smile".
%     \item{\bfseries{Translate:}} Translate emojis into descriptive text or learn emoji representations from their descriptions.
% \end{itemize}

% Research based on replacing or translating emojis prove that extract information in emojis can improve many natural language processing tasks, such as sentiment analysis, machine translation and question and answer systems. The most intuitive way to make use of information hidden in emojis is to learn the representation of emojis just like words. Sanjaya W. proposed a deep learning-based semantic understanding method for emoji, called EmojiNet, which is a dataset containing a large number of Emoji meanings, and by extracting the English meanings from the network and linking of contextual words to provide a machine-readable interpretation of Emoji \cite{emojinet}. Ben E. has proposed a method called emoji2vec. This model learns the representation of emojis from their English descriptions \cite{eisner2016emoji2vec}. Anurag I. has proposed a model that learns emoji embeddings using emoji co-occurrence network graph \cite{illendula2018learning}. Chuchu L. has proposed a model called CEmo-LSTM, uses a Bi-LSTM architecture and is based on an emoji-embedding technique that translates emojis into corresponding sentiment words. The model also takes into account different functions of emojis in texts and classifies posts based on their emoji usage \cite{LIU2021246}.  Choudhary N. proposes a novel method called CESNA to learn emoji-based representations of resource-poor languages by jointly training them with resource-rich languages using a siamese network. The model uses a contrastive loss function based on a similarity metric to project sentences with similar emojis closer to each other and sentences with different emojis farther from each other \cite{10.1007/978-3-031-23804-8_11}. 
% }
